Semistochastic Quadratic Bound Methods

Partition functions arise in a variety of settings, including conditional random fields, logistic regression, and latent gaussian models. In this paper, we consider semistochastic quadratic bound (SQB) methods for maximum likelihood inference based on partition function optimization. Batch methods based on the quadratic bound were recently proposed for this class of problems, and performed favorably in comparison to state-of-the-art techniques. Semistochastic methods fall in between batch algorithms, which use all the data, and stochastic gradient type methods, which use small random selections at each iteration. We build semistochastic quadratic bound-based methods, and prove both global convergence (to a stationary point) under very weak assumptions, and linear convergence rate under stronger assumptions on the objective. To make the proposed methods faster and more stable, we consider inexact subproblem minimization and batch-size selection schemes. The efficacy of SQB methods is demonstrated via comparison with several state-of-the-art techniques on commonly used datasets.

==> Makefile <==
.SUFFIXES: .eps .pdf
LATEX= pdflatex
BIBTEX= bibtex
FIG2DEV=fig2dev

TEX=ElasticCheck.tex \
		parallel.tex \
    ref.bib 

all: pdf 

pdf: $(TEX) ElasticCheck.bbl
	@echo Compiling ElasticCheck
	@$(LATEX) ElasticCheck
	@$(MAKE) fixlabels

fixlabels:
ifneq ($(shell grep -s -c 'Label(s) may have changed. Rerun to get cross-references right.' ElasticCheck.log),0)
	@echo Compiling ElasticCheck again to fix labels
	@$(LATEX) ElasticCheck
else
	@echo " " Labels are correct
endif

ElasticCheck.bbl: ref.bib
	@echo Compiling ElasticCheck for bibliography
	@$(LATEX) ElasticCheck
	@echo Generating bibliography
	@$(BIBTEX) ElasticCheck
	@echo Recompiling ElasticCheck after generating bibliography
	@$(LATEX)  ElasticCheck
	@$(MAKE) fixlabels

.eps.pdf:
	@echo " " Converting $< to $(@F)
	@epstopdf --outfile=Figs/$(@F) $<

clean:
	@echo "Cleaning the figures directory"
	@rm -f figures/*.gpl
	@echo "Cleaning the ElasticCheck directory"
	@rm -f ElasticCheck.pdf ElasticCheck.ps *.aux *.dvi *.log *.bbl *.blg *.toc *.out *.bak

